Technical report: Graph Neural Networks go Grammatical

This paper introduces a framework for formally establishing a connection between a portion of an algebraic language and a Graph Neural Network (GNN). The framework leverages Context-Free Grammars (CFG) to organize algebraic operations into generative rules that can be translated into a GNN layer model. As CFGs derived directly from a language tend to contain redundancies in their rules and variables, we present a grammar reduction scheme. By applying this strategy, we define a CFG that conforms to the third-order Weisfeiler-Lehman (3-WL) test using MATLANG. From this 3-WL CFG, we derive a GNN model, named G$^2$N$^2$, which is provably 3-WL compliant. Through various experiments, we demonstrate the superior efficiency of G$^2$N$^2$ compared to other 3-WL GNNs across numerous downstream tasks. Specifically, one experiment highlights the benefits of grammar reduction within our framework.

==> data/EXPQM9GMNreduct12.tex <==
Target,PPGN,G$^2$N$^2$(16),G$^2$N$^2$(32)
$\mu$,0.231,\textbf{0.127},\textbf{0.102}
$\alpha$,0.382,\textbf{0.268},\textbf{0.196}
$\epsilon_{\mathrm{homo}}$,{0.00276},\textbf{0.00268},{0.0021}
$\epsilon_{\mathrm{lumo}}$,{0.00287},\textbf{0.00268},\textbf{0.00211}
$\Delta\epsilon$,{0.0029},{0.00369},\textbf{0.00287}
$R^2$,16.07,\textbf{1.48},\textbf{1.19}
ZPVE,{0.00064},\textbf{0.000203},\textbf{0.0000151}
$U_0$,{0.234},\textbf{0.0745},\textbf{0.0502}
$U$,{0.234},\textbf{0.0744},\textbf{0.0503}
$H$,{0.229},\textbf{0.0746},\textbf{0.0503}
$G$,{0.238},\textbf{0.0744},\textbf{0.0504}
$C_v$,0.184,\textbf{0.0904},\textbf{0.0707}
T $/$ ep,131 s,27 s, 57 s

==> data/EXPQM9reduct12full.tex <==
Target,PPGN,G$^2$N$^2$(16),G$^2$N$^2$(32),G$^2$N$^2$(64)
$\mu$,0.231,\textbf{0.127},\textbf{0.102},\textbf{0.0703}
$\alpha$,0.382,\textbf{0.268},\textbf{0.196},\textbf{0.127}
$\epsilon_{\mathrm{homo}}$,{0.00276},\textbf{0.00268},{0.0021},\textbf{0.00172}
$\epsilon_{\mathrm{lumo}}$,{0.00287},\textbf{0.00268},\textbf{0.00211},\textbf{0.00153}
$\Delta\epsilon$,{0.0029},{0.00369},\textbf{0.00287},\textbf{0.00253}
$R^2$,16.07,\textbf{1.48},\textbf{1.19},\textbf{0.342}
ZPVE,{0.00064},\textbf{0.000203},\textbf{0.0000151},\textbf{0.0000951}
$U_0$,{0.234},\textbf{0.0745},\textbf{0.0502},\textbf{0.0169}
$U$,{0.234},\textbf{0.0744},\textbf{0.0503},\textbf{0.0162}
$H$,{0.229},\textbf{0.0746},\textbf{0.0503},\textbf{0.0176}
$G$,{0.238},\textbf{0.0744},\textbf{0.0504},\textbf{0.0214}
$C_v$,0.184,\textbf{0.0904},\textbf{0.0707},\textbf{0.0429}
Time $/$ epoch,131 s,27 s, 57 s, 102 s
